Edge Computing in IoT: A 6G Perspective

Edge computing is one of the key driving forces to enable Beyond 5G (B5G) and 6G networks. Due to the unprecedented increase in traffic volumes and computation demands of future networks, multi-access (or mobile) edge computing (MEC) is considered as a promising solution to provide cloud-computing capabilities within the radio access network (RAN) closer to the end users. There has been a significant amount of research on MEC and its potential applications; however, very little has been said about the key factors of MEC deployment to meet the diverse demands of future applications. In this article, we present key considerations for edge deployments in B5G/6G networks including edge architecture, server location and capacity, user density, security etc. We further provide state-of-the-art edge-centric services in future B5G/6G networks. The paper also present experimental evaluation of edge-based services deployment including video transcoding and deep learning inference. Lastly, we present some interesting insights and open research problems in edge computing for 6G networks.

==> tab_mec1.tex <==
%--------------------------------------------  Table ----------------------------------
% There is something seriously confusing in this table. The first column entries should be
% Normally complete sentences should be avoided to save space in such table.

\begin{table*}[h!]
\centering
\small
\caption{\label{tab:mec1}Edge considerations for key B5G/6G use cases.}

 \begin{tabular}{ >{\columncolor{airforceblue!40}}m{3cm} >{\columncolor[gray]{0.9}}m{2.5cm} >{\columncolor{airforceblue!40}}m{2.5cm}  >{\columncolor[gray]{0.9}}m{2.5cm}  >{\columncolor{airforceblue!40}}m{2.5cm} >{\columncolor[gray]{0.9}}m{2.5cm} } 
 
 \textbf{Edge Considerations} & \textbf{Video Analytics} & \textbf{ITS} &\textbf{Manufacturing} & \textbf{Energy} & \textbf{Agriculture} \\ [0.5em] 
 \hline
 
 % Asif: What is the difference b/w MEC equipment, MEC centers and other cells etc.. Its not clear to me.
 % Mariam: Revised
 Applications & Object detection, tracking, AR/VR  &Autonomous cars, UAVs & Robots and drones, Automated guided vehicles (AGVs) & Virtual Power Plant (VPP), Smart grid & Sensors, Drones \\[1em] \arrayrulecolor{gray!50}\hline

% Architecture \cite{gsma2020} & China Unicom is using MEC and mobile networks to deploy fully connected, low-latency and high-bandwidth networks. & China Telecom is adopting cloud-based 5G core and MEC to support Internet of vehicles. & China Mobile is supporting a 5G-connected MEC architecture.
%  & ZTE is offering a convergent fixed and mobile network solution with MEC capabilities to support smart grids. & Huawei’s 5G MEC with application-centric edge computing and adjustable network resources. \\[1em] \arrayrulecolor{gray!50}\hline

Architecture \cite{gsma2020} & China Unicom is using MEC and mobile networks to deploy fully connected, low-latency and high-bandwidth networks. & China Telecom is adopting cloud-based 5G core and MEC to support Internet of vehicles. & China Mobile is supporting a 5G-connected MEC architecture.
 & ZTE is offering a convergent fixed and mobile network solution with MEC capabilities to support smart grids. & Huawei’s 5G MEC with application-centric edge computing and adjustable network resources. \\[1em] \arrayrulecolor{gray!50}\hline
 
 % Asif: Why 1 ms (very low) for agriculture use cases?
 % Mariam: Corrected
Latency \cite{huawei} & 2-10 ms & $<$10 ms & $<$1 ms  & 10 ms & 10 ms \\[1em] \arrayrulecolor{gray!50}\hline

%Capacity \cite{xyz} & aaa & bbb & ccc & ddd & eee \\[0.5pt] \arrayrulecolor{gray!50}\hline
 
Edge location \cite{gsma2020} & Centralized data center in network facility by Verizon & One data center per specified location & One data center per specified location & Specified locations in Network Cloud & Specified locations in Network Cloud \\[1em] \arrayrulecolor{gray!50}\hline


\begin{comment}
%% Asif: The following row needs to changed/deleted. i.e.,
% FL is just one of many algorithms to bring intelligence at the edge. this covers a lot whole of the ML/DL algorithms. Also check the Ref is not present in .bib file.
% \cite{A}, Put a Ref.
% Mariam: Reference added
Intelligence \cite{xia2021}& \red{Image classification and segmentation using federated learning} & \red{Mobility management through edge federated learning} & Federated learning & Federated energy demand learning & Federated learning \\[1em] \arrayrulecolor{gray!50}\hline
\end{comment}

%% Asif: It could be something e.g., MEC Real world Deployments (if it is).
% Mariam: Yes, rephrased. Given reference is applicable to all columns
Security and Privacy in real world deployments of MEC \cite{5Gensure} & 5G-ENSURE  & 5G-ENSURE & SONATA  & COGNET  & 5G-ENSURE  \\[1em] \arrayrulecolor{gray!50}\hline

Device Density Worth \cite{huawei} & $>$US{\$} 4 billion & 60.3 million devices & Annual growth rate of 464 {\%} & US{\$} 36 billion & US{\$} 33.9 billion \\[1ex] 
%  \hline
 \end{tabular}
\end{table*}
%------------------------------------------------------------------------------


==> tab_mec3.tex <==

\begin{table*}[h!]
\centering
\small
% \renewcommand{\arraystretch}{0.9}
\caption{\label{tab:mec3}Summary of recent surveys using Edge Computing for IoT.}
 \begin{tabular}{ >{\columncolor{airforceblue!40}}m{1.5cm} >{\columncolor[gray]{0.9}}m{10cm} >{\columncolor{airforceblue!40}}m{4cm} } 
 
 \textbf{Ref, Year} & \textbf{Main Contribution} & \textbf{Application Area(s)} \\ [0.5em] 
 \arrayrulecolor{white}\hline


%% 1 
\cite{survey1}, 2021 &The paper surveys the data and connectivity requirements of a smart city using 5G. It is shown how cloud computing alone cannot serve this requirement and provides a framework using MEC operative in smart city environment. & Smart city \\[1em] %\arrayrulecolor{gray!50}\hline
 
 
%% 2 
\cite{survey2}, 2021    &The paper presents a detailed overview of Intelligence Edge Computing (IEC) in 5G and foresees its characteristics, challenges, potential use cases and market drivers for 6G.    &Customer oriented services, Operator and third-party services\\[1em] %\arrayrulecolor{gray!50}\hline

%% 3 
\cite{survey3}, 2021  &A survey on recent advances in enabling technologies for E2E network slicing and current standardization efforts in 5G and a vision for 6G has been presented.   &Generic 5G use cases, e-health, V2X \\[1em] %\arrayrulecolor{gray!50}\hline

%% 4 
\cite{survey4}, 2021 &The security vulnerabilities of 5G use cases deployed in accordance to MEC-based scenarios have been surveyed in this paper.   &Critical infrastructure-based services, Machine-to-Machine (M2M), V2V, Augmented Reality (AR)/ Virtual Reality (VR)  \\[1em] %\arrayrulecolor{gray!50}\hline


 \end{tabular}
\end{table*}
%------------------------------------------------------------------------------

